Identification of parameters in the torsional dynamics of a drilling process through Bayesian statistics

This work presents the estimation of the parameters of an experimental setup, which is modeled as a system with three degrees of freedom, composed by a shaft, two rotors, and a DC motor, that emulates a drilling process. A Bayesian technique is used in the estimation process, to take into account the uncertainties and variabilities intrinsic to the measurement taken, which are modeled as a noise of Gaussian nature. With this procedure it is expected to check the reliability of the nominal values of the physical parameters of the test rig. An estimation process assuming that nine parameters of the experimental apparatus are unknown is conducted, and the results show that for some quantities the relative deviation with respect to the nominal values is very high. This deviation evidentiates a strong deficiency in the mathematical model used to describe the dynamic behavior of the experimental apparatus.

==> Makefile <==
##############################################################################
#
# Makefile for LaTeX files
# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile
# First modification by Matti Airas <Matti.Airas@hut.fi>
# Second modification by Thomas Lewiner <lewiner@gmail.com>
# Third modification by Americo Barbosa da Cunha Jr <americo.cunhajr@gmail.com>
# last update: Jan 4, 2010
#
##############################################################################


######################### Programs ################################

#LATEX	  = pdflatex --shell-escape -interaction=nonstopmode
LATEX	  = latex -src-specials -interaction=nonstopmode
BIBTEX	  = bibtex
MAKEINDEX = makeindex
XDVI	  = xdvi -gamma 4
DVIPS	  = dvips
DVIPDF    = dvipdfm
L2H	  = latex2html -split 0
TTH	  = tth #-a -e2
GH	  = gv
XPDF	  = xpdf
RM        = rm -Rf


########################## Sources ################################

# BEGIN DEPENDENCIES

SRC       := msc_mario_sandoval.tex
CLASSES   := puc-rio_tese.cls
STYLES    := atbeginend.sty chngpage.sty nomencl.sty
INPUTS    := *.tex
BIBFILE   := bibliografia.bib
BIBSTYLES := puc-rio_num_br.bst puc-rio_bib_br.bst
INPUTENCS := noaccent.def
EPSPICS   := puc_logo.eps

# END DEPENDENCIES


DVI	 = $(SRC:%.tex=%.dvi)
PSF	 = $(SRC:%.tex=%.ps)
PDF	 = $(SRC:%.tex=%.pdf)
HTM	 = $(SRC:%.tex=%_htm)
HTML	 = $(SRC:%.tex=%.html)


####################### Dependencies ##############################


ifeq ($(MAKECMDGOALS),depend)

SRC     := $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)

CLASSES := $(shell perl -ne '($$_)=/^[^%]*\\documentclass[^{]*\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.cls "}' $(SRC))
CLASSES := $(sort $(foreach class,$(CLASSES), $(shell if [ -f $(class) ] ; then echo $(class) ; else echo class $(class) not in folder >&2 ; fi ;) ) )

STYLES  := $(shell perl -ne '($$_)=/^[^%]*\\[useRqir]+[Pp]ackage[^{]*\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.sty "}' $(SRC) $(CLASSES))
STYLES  := $(sort $(foreach style,$(STYLES), $(shell if [ -f $(style) ] ; then echo $(style) ; else echo style $(style) not in folder >&2 ; fi ;) ) )

BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
BIBFILE := $(sort $(foreach bibfile,$(BIBFILE), $(shell if [ -f $(bibfile) ] ; then echo $(bibfile) ; else echo bibfile $(bibfile) not in folder >&2 ; fi ;) ) )

BIBSTYLES := $(shell perl -ne '($$_)=/^[^%]*\\bibliographystyle[^{]*\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bst "}' $(SRC) $(INPUTS) $(CLASSES) $(STYLES))
BIBSTYLES := $(sort $(foreach bibstyle,$(BIBSTYLES), $(shell if [ -f $(bibstyle) ] ; then echo $(bibstyle) ; else echo bibstyle $(bibstyle) not in folder >&2 ; fi ;) ) )

INPUTS  := $(shell perl -ne '($$_)=/^[^%]*\\input\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.tex "}' $(SRC) $(CLASSES) $(STYLES) $(BIBSTYLES) )
INPUTS  := $(sort $(foreach input,$(INPUTS), $(shell if [ -f $(input) ] ; then echo $(input) ; else echo input file $(input) not in folder >&2 ; fi ;) ) )

INPUTENCS := $(shell perl -ne '($$_)=/^[^%]*\\inputencoding\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.def "}' $(SRC) $(CLASSES) $(STYLES) $(BIBSTYLES) )
INPUTENCS := $(sort $(foreach inputenc,$(INPUTENCS), $(shell if [ -f $(inputenc) ] ; then echo $(inputenc) ; else echo inputenc $(inputenc) not in folder >&2 ; fi ;) ) )

EPSPICS := \
  $(shell perl -ne '($$_)=/^[^%]*\\includegraphics[^{}]*\{([^@\#]*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b "}' $(SRC) $(INPUTS) $(CLASSES) $(STYLES) $(BIBSTYLES) ) \
  $(shell perl -ne '($$_)=/^[^%]*\\[tvsingleubo]+image[{[].*\{([^{}]*?)\}/;@_=split /,/;foreach $$b (@_) {print "figs/$$b "}' $(SRC) $(INPUTS) ) \
  $(shell perl -ne '($$_)=/^[^%]*\\watermark[^{}]*\{([^{}]*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b "}' $(SRC) $(INPUTS) ) \
  $(shell perl -ne '($$_)=/^[^%]*\\logouni[^{}]*\{([^{}]*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b "}' $(SRC) $(INPUTS) )
EPSPICS := $(sort $(foreach fig,$(EPSPICS), $(shell if [ -f $(fig) ] ; then echo $(fig) ; else if [ -f $(fig).eps ] ;  then echo $(fig).eps ; else if [ -f $(fig).ps ] ;  then echo $(fig).ps ; else if [ -f $(fig).png ] ;  then echo $(fig).png ; else echo figure $(fig) not in folder >&2 ; fi ; fi ; fi ; fi ;) ) )

endif


######################### Messages ################################

RERUN     = "(!|(There were undefined references|Rerun to get (cross-references|the bars) right))"
RERUNBIB  = "No file.*\.bbl|Citation.*undefined"
MAKEIDX   = "^[^%]*\\makeindex"
MPRINT    = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"
OUTDATED  = echo "EPS-file is out-of-date!" && false


########################## Macros #################################

define run-latex
	if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi && \
	if test -r $(<:%.tex=%.idx); then cp $(<:%.tex=%.idx) $(<:%.tex=%.idx.bak); fi && \
	$(LATEX) $< > /dev/null ; true
endef


define rerun-latex
	if cmp -s $(<:%.dvi=%.tex) $(<:%.dvi=%.tex.bak) ; \
	  then rm $(<:%.dvi=%.tex.bak) ; \
	  else \
	    touch -r $(<:%.dvi=%.tex) $(<:%.dvi=%.tex.bak) ; \
	    mv $(<:%.dvi=%.tex.bak) $(<:%.dvi=%.tex) ; \
	    $(run-latex) ; \
	    touch -r $(<:%.dvi=%.tex) $< ; \
	fi
endef


define run-complete
	$(run-latex)
    $(MAKEINDEX) $(SRC:%.tex=%.nlo) -s nomencl.ist -o $(SRC:%.tex=%.nls)
	( egrep -q $(MAKEIDX) $< > /dev/null && \
    ! (cmp -s $(<:%.tex=%.idx) $(<:%.tex=%.idx.bak)) ) && ( \
    $(MAKEINDEX) $(<:%.tex=%) 2>&1 | egrep -i "(lines|error)" ; $(run-latex) ) ; true
	( for file in $(BIBFILE) ; do if [ $file -nt $(<:%.tex=%.bbl) ] ; then \
    $(BIBTEX) $(<:%.tex=%) | egrep -i "(Database|error)" ; $(run-latex) ; break ; fi; done ; ) ; true
  ( egrep -q $(RERUNBIB) $(<:%.tex=%.log) > /dev/null && \
    $(BIBTEX) $(<:%.tex=%) | egrep -i "(Database|error)" ; $(run-latex) ) ; true
	egrep -q $(RERUN) $(<:%.tex=%.log) > /dev/null && $(run-latex) ; true
	egrep -q $(RERUN) $(<:%.tex=%.log) > /dev/null && $(run-latex) ; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak) ; then true ; else $(run-latex) ; fi
	$(RM) $(<:%.tex=%.toc.bak) $(<:%.tex=%.idx.bak)
endef


define show-warnings
	if test -e $(<:%.tex=%.blg) ; then \
    egrep -B1 -A3 -i "line " $(<:%.tex=%.blg) ; \
	  egrep -i "Warning-" $(<:%.tex=%.blg) ; \
  fi ; true
	if test -e $(<:%.tex=%.log) ; then \
    egrep -i "Overful" $(<:%.tex=%.log) ; \
    egrep -i "Warning" $(<:%.tex=%.log) ; \
    egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; \
    egrep -A3 -i "^!" $(<:%.tex=%.log) ; \
  fi ; true
endef

define show-stats
	if test -e $(<:%.tex=%.ilg) ; then \
    echo -n "Index  : " ; egrep -i "Generating" $(<:%.tex=%.ilg) ; \
  fi ; true
	if test -e $(<:%.tex=%.blg) ; then \
    echo -n "BibTeX : " ; egrep -i "entries" $(<:%.tex=%.blg) ; \
  fi ; true
	if test -e $(<:%.tex=%.log) ; then \
	  echo -n "LaTeX  : " ; egrep -i "written" $(<:%.tex=%.log) ; \
  fi ; true
	if test -e $(<:%.tex=%.aux) ; then \
    echo -n "         " ; \
    echo -n $(shell egrep -c "contentsline {chapter}" $(<:%.tex=%.aux)) ; echo -n " chapters, " ; \
    echo -n $(shell egrep -c "contentsline {section}" $(<:%.tex=%.aux)) ; echo -n " sections and, " ; \
    echo -n $(shell egrep -c "contentsline {subsection}" $(<:%.tex=%.aux)) ; echo " subsections." ; \
  fi ; true
endef


####################### File Targets ##############################

dvi	 : $(DVI)

ps	 : $(PSF) 

pdf	 : $(PDF) 

htm	 : $(HTM)

html : $(HTML)

DIRNAME = $(notdir ${PWD})
TARNAME = ../$(shell echo $(DIRNAME) | tr [:upper:] [:lower:]).tgz
tar  : $(TARNAME)


###################### default targets ############################

all 	  :
	make depend
	@for i in $(DVI) ; do if egrep -q -i $(RERUN) $${i/.dvi/.log} ; then $(RM) $$i ; fi ; done ; true
	make dvi

everything :
	make depend
	@for i in $(DVI) ; do if egrep -q -i $(RERUN) $${i/.dvi/.log} ; then $(RM) $$i ; fi ; done ; true
	make dvi
	@for i in $(PSF) $(PDF) $(HTML) $(HTM) ; do if test -r $$i ; then make $$i ; fi ; done ; true
	make tar
	make cvs

.PHONY	: all everything depend warns stats show-depend clean dvi ps pdf htm html show showps showpdf tar cvs


##################### Programs Targets ############################

show	: $(DVI)
	@for i in $(DVI) ; do $(XDVI) $$i ; done

showps	: $(PSF)
	@for i in $(PSF) ; do $(GH) $$i ; done

showpdf	: $(PDF)
	@for i in $(PDF) ; do $(XPDF) $$i ; done

clean	:
	$(RM) .\#* *~ $(DVI) $(PSF) $(PDF) $(HTM) $(HTML) \
  $(DVI:%.dvi=%.aux) $(DVI:%.dvi=%.log) $(DVI:%.dvi=%.out) \
  $(DVI:%.dvi=%.bbl) $(DVI:%.dvi=%.blg) $(DVI:%.dvi=%.brf) \
  $(DVI:%.dvi=%.lof) $(DVI:%.dvi=%.lot) $(DVI:%.dvi=%.toc) \
  $(DVI:%.dvi=%.idx) $(DVI:%.dvi=%.ilg) $(DVI:%.dvi=%.ind) \
  $(DVI:%.dvi=%.tid) $(DVI:%.dvi=%.tin) $(DVI:%.dvi=%.tms)

cvs :
	cvs ci -m "backup $(shell date -u '+%A, %d %b %Y, %H:%M')"


####################### Info Targets ##############################

warns	: $(SRC)
	  @$(show-warnings)

stats	: $(SRC)
	  @$(show-stats)

show-depend :
	  @echo "# sources   : " $(SRC)
	  @echo "# classes   : " $(CLASSES)
	  @echo "# styles    : " $(STYLES)
	  @echo "# inputs    : " $(INPUTS)
	  @echo "# biblios   : " $(BIBFILE)
	  @echo "# bibstyles : " $(BIBSTYLES)
	  @echo "# encodings : " $(INPUTENCS)
	  @echo "# images    : " $(EPSPICS)

depend :
	  @rm -f Makefile.bak*
	  @csplit Makefile -s -f Makefile.bak "/^\# BEGIN DEPENDENCIES/2" "/^\# END DEPENDENCIES/-1"
	  @rm -f Makefile.bak01
	  @echo > Makefile.bak01
	  @echo "SRC       := $(SRC)      "  > Makefile.bak01
	  @echo "CLASSES   := $(CLASSES)  " >> Makefile.bak01
	  @echo "STYLES    := $(STYLES)   " >> Makefile.bak01
	  @echo "INPUTS    := $(INPUTS)   " >> Makefile.bak01
	  @echo "BIBFILE   := $(BIBFILE)  " >> Makefile.bak01
	  @echo "BIBSTYLES := $(BIBSTYLES)" >> Makefile.bak01
	  @echo "INPUTENCS := $(INPUTENCS)" >> Makefile.bak01
	  @echo "EPSPICS   := $(EPSPICS)  " >> Makefile.bak01
	  @cat Makefile.bak00 Makefile.bak01 Makefile.bak02 > Makefile.bak
	  @rm -f Makefile.bak0*
	  @mv Makefile.bak Makefile
	  @make show-depend


###################### File generation ############################

$(DVI)	: %.dvi : %.tex $(INPUTS) $(DEP) $(BIBFILE) $(INPUTENCS) $(EPSPICS) $(CLASSES) $(STYLES) $(BIBSTYLES)
	@$(run-complete)
	@$(show-warnings)
	@echo ; true
	@$(show-stats)

$(PSF)	: %.ps : %.dvi
	@sed -e "s/[[]dvipdfm[]]/[dvips]/g" $(<:%.dvi=%.tex) > $(<:%.dvi=%.tex.bak)
	@$(rerun-latex)
	@$(DVIPS) $< -o $@

$(PDF)  : %.pdf : %.dvi
	@sed -e "s/[[]dvips[]]/[dvipdfm]/g" $(<:%.dvi=%.tex) > $(<:%.dvi=%.tex.bak)
	@$(rerun-latex)
	@$(DVIPDF) -o $@ $<

$(HTML)	:	%.html : %.tex $(DEP)
	@$(TTH) $<

$(HTM)	:	%_htm : %.tex $(DEP) $(BIBFILE)
	mkdir -p $@
	@$(L2H) -dir $@ $(SRC)
	touch -r $< $@

$(TARNAME) : $(SRC) $(DVI:%.dvi=%.bbl) $(DVI:%.dvi=%.pdf) $(CLASSES) $(STYLES) $(INPUTS) $(BIBFILE) $(BIBSTYLES) $(INPUTENCS) $(EPSPICS) Makefile figs/*.[^e][^p][^s]
	tar -C.. -c -v -z --exclude=CVS -f $@ $(foreach file,$^,$(DIRNAME)/$(file)) > /dev/null

